An Intermediate Representation for Composable Typed Streaming Dataflow Designs

Tydi is an open specification for streaming dataflow designs in digital circuits, allowing designers to express how composite and variable-length data structures are transferred over streams using clear, data-centric types. These data types are extensively used in a many application domains, such as big data and SQL applications. This way, Tydi provides a higher-level method for defining interfaces between components as opposed to existing bit and byte-based interface specifications. In this paper, we introduce an open-source intermediate representation (IR) which allows for the declaration of Tydi's types. The IR enables creating and connecting components with Tydi Streams as interfaces, called Streamlets. It also lets backends for synthesis and simulation retain high-level information, such as documentation. Types and Streamlets can be easily reused between multiple projects, and Tydi's streams and type hierarchy can be used to define interface contracts, which aid collaboration when designing a larger system. The IR codifies the rules and properties established in the Tydi specification and serves to complement computation-oriented hardware design tools with a data-centric view on interfaces. To support different backends and targets, the IR is focused on expressing interfaces, and complements behavior described by hardware description languages and other IRs. Additionally, a testing syntax for the verification of inputs and outputs against abstract streams of data, and for substituting interdependent components, is presented which allows for the specification of behavior. To demonstrate this IR, we have created a grammar, parser, and query system, and paired these with a backend targeting VHDL.

==> sections/02_keywords.tex <==
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010583.10010682.10010689</concept_id>
       <concept_desc>Hardware~Hardware description languages and compilation</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010583.10010633.10010645</concept_id>
       <concept_desc>Hardware~Design reuse and communication-based design</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010583.10010717.10010721.10010726</concept_id>
       <concept_desc>Hardware~Transaction-level verification</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Hardware~Hardware description languages and compilation}
\ccsdesc[500]{Hardware~Design reuse and communication-based design}
\ccsdesc[300]{Hardware~Transaction-level verification}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{hardware description languages, intermediate representations, open source software, hardware streams, data structures}

==> sections/20_body/50_collaboration.tex <==
\subsection{Documentation}
\todo{Elaborate on how "documentation" is an actual node in the IR, in addition to conventional comments. Backends can propagate documentation to their generated code.}

\subsection{Project Structure}
\todo{Simple, minimal project file which specifies file locations (relative paths) and compiler options. Suitable for version control.}

\subsection{Reuse}
\todo{Project imports, allow for importing types, interfaces, implementations...}

==> sections/80_acknowledgements.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
\todo{Acknowledgements?}

\todo{Remove todonotes package after finishing. (Not in list of approved packages, so just to be sure even when all the todos are done.)}

% \todo{NOTE: One (separate?) page of references is allowed, and does not count towards the 8-page total: \url{https://iccad.com/scientific-paper/}}
\end{acks}
